Reasoning in the OWL 2 Full Ontology Language using First-Order Automated Theorem Proving

OWL 2 has been standardized by the World Wide Web Consortium (W3C) as a family of ontology languages for the Semantic Web. The most expressive of these languages is OWL 2 Full, but to date no reasoner has been implemented for this language. Consistency and entailment checking are known to be undecidable for OWL 2 Full. We have translated a large fragment of the OWL 2 Full semantics into first-order logic, and used automated theorem proving systems to do reasoning based on this theory. The results are promising, and indicate that this approach can be applied in practice for effective OWL reasoning, beyond the capabilities of current Semantic Web reasoners. This is an extended version of a paper with the same title that has been published at CADE 2011, LNAI 6803, pp. 446-460. The extended version provides appendices with additional resources that were used in the reported evaluation.

==> resources/DoGNUPlot <==
set terminal postscript eps
set output "fig-results-fullish-orderedtimes.eps"
# set output "/home/graph/tptp/public_html/Guest/fig-results-fullish-orderedtimes.eps"
set style data linespoints
# set title "Full-characteristics Test Cases"
set xlabel "Solution number"
set ylabel "CPU time in seconds (log scale)" 2
set key 12,250
set grid
# set offsets 0,0,1.200000,1.200000
set logscale y
set size 1,0.5
plot [1:32] [0.008:300] \
"data-fullish" using 1:2 title "Vampire Small" ,\
"data-fullish" using 1:3 title "iProver-SInE Small" ,\
"data-fullish" using 1:4 title "Vampire Complete" ,\
"data-fullish" using 1:5 title "iProver-SInE Complete"

set terminal postscript eps
set output "fig-results-bulk-orderedtimes.eps"
# set output "/home/graph/tptp/public_html/Guest/fig-results-bulk-orderedtimes.eps"
set style data linespoints
# set title "Full-characteristics Test Cases"
set xlabel "Solution number"
set ylabel "CPU time in seconds (log scale)" 2
set key 16,250
set grid
# set offsets 0,0,1.200000,1.200000
set logscale y
set size 1,0.5
plot [1:32] [10:300] \
"data-fullish" using 1:6 title "Vampire Small" ,\
"data-fullish" using 1:7 title "Vampire-SInE Small" ,\
"data-fullish" using 1:8 title "iProver-SInE Small" ,\
"data-fullish" using 1:9 title "Vampire Complete" ,\
"data-fullish" using 1:10 title "Vampire-SInE Complete" ,\
"data-fullish" using 1:11 title "iProver-SInE Complete"

set terminal postscript eps
set output "fig-results-coverage-orderedtimes.eps"
# set output "/home/graph/tptp/public_html/Guest/fig-results-coverage-orderedtimes.eps"
set style data linespoints
# set title "Full-characteristics Test Cases"
set xlabel "Solution number"
set ylabel "CPU time in seconds (log scale)" 2
set key 100,280
set grid
# set offsets 0,0,1.200000,1.200000
set logscale y
set size 1,0.5
plot [1:411] [0.01:500] \
"data-coverage" using 1:2 title "Vampire" ,\
"data-coverage" using 1:3 title "iProver-SInE"


==> resources/tab-results-coverage-atp-small.tex <==
\begin{tabular}{|l||r|r|r|}
\hline
\textbf{Reasoner} & 
\textbf{Success} & 
\textbf{Wrong} & 
\textbf{Unknown} \\ 
\hline
\hline
iProver-SInE
& 396 & 0 & 15 \\
\hline
\end{tabular}

